Backstepping Reach-avoid Controller Synthesis for Multi-input Multi-output Systems with Mixed Relative Degrees

Designing controllers with provable formal guarantees has become an urgent requirement for cyber-physical systems in safety-critical scenarios. Beyond addressing scalability in high-dimensional implementations, controller synthesis methodologies separating safety and reachability objectives may risk optimization infeasibility due to conflicting constraints, thereby significantly undermining their applicability in practical applications. In this paper, by leveraging feedback linearization and backstepping techniques, we present a novel framework for constructing provable reach-avoid formal certificates tailored to multi-input multi-output systems. Based on this, we developed a systematic synthesis approach for controllers with reach-avoid guarantees, which ensures that the outputs of the system eventually enter the predefined target set while staying within the required safe set. Finally, we demonstrate the effectiveness of our method through simulations.

==> introduction.tex <==
\section{Introduction}

% Motivation: Backstepping+ Feedback linearization + Reach-avoid Controller Synthesis

% To synthesize reach-avoid controllers for high-dimensional systems, especially when the reach-avoid constraints are defined for the output of the system, to narrow the gap between theory and applications.


The escalating complexity of CPS in real-world applications, coupled with their need to accomplish more sophisticated tasks, is imposing stricter formal requirements on controller design methodologies for modern control systems, particularly in safety-critical scenarios.
In such contexts, controllers must not only avoid unsafe states but also steer the system to achieve the predefined objectives.
This dual requirement, which necessitates formal guarantees that systems initialized from safe configurations will persistently maintain safety until achieving designated goals, has positioned the synthesis of controllers guaranteeing reach-avoid property as a pivotal research focus within the control community.

A prominent methodology for achieving formal guarantees involves designing energy-like value functions that quantify the deviation of a system's behaviors from desired requirements, thereby enabling real-time evaluation of safety or stability violations.
Due to their straightforward integration as additional constraints into specific control problem frameworks such as model predictive control (MPC), such approaches have emerged as a key paradigm for synthesizing controllers with formal guarantees in recent years.
Among these developments, control Lyapunov functions (CLFs) and control barrier functions (CBFs) stand out as the most noteworthy methods for their mathematical rigor and compatibility with real-time optimization, and make them pivotal for safety-critical control in robotics, power systems, and beyond.
This has further led to the unification of CLFs and CBFs through quadratic program (QP) frameworks, enabling the achievement of control objectives while adhering to conditions that ensure the system stays within the safe set.
However, a significant challenge for applying these approaches lies in identifying suitable value functions to serve as corresponding formal certificates, particularly barrier functions to ensure safety.
% , often presents a significant challenge.
While computational techniques such as SOS optimization and Hamilton-Jacobi reachability analysis have demonstrated their applicability in lower-dimensional systems, their scalability limitations motivate ongoing research for complex high-dimensional systems.
% For lower-dimensional systems, computational techniques including sum-of-squares (SOS) optimization and Hamilton-Jacobi reachability analysis have emerged as effective solutions, enabling systematic construction of these certificates while maintaining tractability.
Recent advances such as backstepping-based formal certificate construction approaches have significantly enhanced the scalability of these methodologies when establishing formal guarantees for high-dimensional dynamical systems. \textcolor{red}{(for instance, backstepping + CLF, backstepping + CBF)} The main limitations of these methods are the structural requirements of the dynamics and controllability assumptions, which prevent direct applicability to systems that lack cascaded architecture.
% High order CBFs (HOCBFs), which also establish forward invariance guarantees for safe ..., recursively differentiate safety constraints until control inputs explicitly appear in the derivatives, and then apply CBF-inspired constraints on the highest-order derivatives, thereby eliminates the structural requirements by backstepping methods.
While high order CBFs (HOCBFs) similarly construct a safe set within the set defined by the prescribed constraints to ensure forward invariance, they recursively differentiate safety constraints until control inputs explicitly encoded in the highest-order derivatives, and then apply CBF-inspired conditions on these derivatives, thereby eliminates the structural requirements of backstepping methods under the assumption of uniform relative degree.
This conceptual alignment with feedback linearization has inspired synthesizing control barrier functions for partially feedback linearizable systems \cite{cohen2024constructive}, enabling their deployment in underactuated robotic systems.
However, these frameworks that treat safety and stability formal guarantees as separate certificates may risk computational infeasibility during optimization due to inherent conflicts between these constraints.
In contrast, recent developments in optimization-based reach-avoid controller synthesis propose a unified methodology \cite{xue2024reach} to address this challenge. This approach originates from the characterization of the reach-avoid set \cite{xue2023reach} through the zero-level set of the synthesized value functions, which verifies system compliance with reachability and safety requirements. Beyond simplifying design procedures by eliminating redundant value functions, this method can ensure persistent provable reach-avoid guarantees throughout the evolving of the dynamics, thereby preventing the infeasibility of the problem due to constraint conflicts during the optimization.

In practice, MIMO systems are quite common in daily life and safety constraints are often imposed on observable outputs rather than system states. Motivated by this output-to-state relationship and aforementioned challenges, we in this letter present a systematic reach-avoid controller synthesis framework for MIMO systems. Our main contributions can be summarized as follows.
\begin{itemize}
    \item We propose a constructive framework for generating formal reach-avoid certificates in MIMO systems with uniform relative degrees, and derive a systematic synthesis methodology for controllers that guarantee reach-avoid specifications.
    \item Furthermore, we generalize this framework to address MIMO systems with mixed relative degrees and element-wise output constraints. Building upon this foundation, we establish a reach-avoid controller synthesis approach and rigorously characterize its feasibility conditions.
\end{itemize}
% \begin{itemize}
%     \item We propose a framework for constructing provable reach-avoid formal certificates for MIMO systems with a uniform relative degree. Based on this formal certificate, we then present a systematic controller synthesizing method with reach-avoid formal guarantees.
%     \item Furthermore, we extend the aforementioned formal certificates construction framework to MIMO systems with mixed relative degrees and element-wise constraints on their outputs. We then establish the reach-avoid controller synthesizing approach and discuss the condition for its feasibility.
% \end{itemize}

==> related_work.tex <==
\section{Related work}

\textit{Nonlinear backstepping}

As systems become more complex and engaging mixed order of relative degrees, it is often beneficial to begin the control design process with a simplified high-level model that informs the design of subsystems handling the complete system dynamics. Backstepping is a well-established method for this purpose \cite{vaidyanathan2020backstepping}.



Backstepping has been widely used in safety-critical control to stabilise systems while enforcing constraints. Kim et al. \cite{kim2023safe} developed a safe controller for an under-actuated multicopter using CBF backstepping, while Koga et al. \cite{koga2023safe} proposed a backstepping QP controller with safety constraints. Taylor et al. utilise backstepping approach to construct CBF for systems with potentially mixed high relative degree \cite{taylor2022safe}.
These approaches ensure safe operation by structuring the controller to establish a linear dynamic relationship between sequential states in cascade, allowing the system to satisfy safety requirements as it stabilises. 


Other methods to design safety-critical stabilising controller for high-order nonlinear systems:

exponential approach, for example the exponential barrier function \cite{nguyen2016exponential, nguyen2021robust},

high-order control barrier function, by constructing sublevel set for each derivative layer \cite{xiao2019control,xiao2021high}.




\textit{Feedback linearisation}


In this paper, we use the structure derived from feedback linearisation \cite{khalil2002nonlinear} to aid the backstepping-based synthesis of a reach-avoid controller.


(Xiangru X)\cite{xu2018constrained} \cite{abel2023prescribed} treating safety constraints directly as outputs for strict-feedback nonlinear systems.


Cohen et al. used the cascaded structure of feedback linearisation to construct valid barrier functions for nonlinear systems \cite{cohen2024constructive}.


\textit{Reach-avoid}


Learning safe, generalisable perception-based reach-avoid \cite{dawson2022learning}.

Controller synthesis for linear systems with reach-avoid specification \cite{fan2018controller} \cite{fan2021controller}.

CBF reach-avoid, combining CBF with HJR, computationally expensive \cite{choi2021robust}

Reach-avoid problem with time varying dynamics, targets and constraints \cite{fisac2015reach}.

Reach-avoid via reinforcement learning \cite{hsu2021safety}.

\cite{deka2018robust} proposed a method that uses state feedback in the joint space of robot manipulators, but has a limitation of extending to more general geometry.

\cite{chen2025distributionally} use SOS solved for barrier certificate, safety guarantees for stochastic control systems.


\textcolor{red}{TODO}
